Towards a Common Understanding of Contributing Factors for Cross-Lingual Transfer in Multilingual Language Models: A Review

In recent years, pre-trained Multilingual Language Models (MLLMs) have shown a strong ability to transfer knowledge across different languages. However, given that the aspiration for such an ability has not been explicitly incorporated in the design of the majority of MLLMs, it is challenging to obtain a unique and straightforward explanation for its emergence. In this review paper, we survey literature that investigates different factors contributing to the capacity of MLLMs to perform zero-shot cross-lingual transfer and subsequently outline and discuss these factors in detail. To enhance the structure of this review and to facilitate consolidation with future studies, we identify five categories of such factors. In addition to providing a summary of empirical evidence from past studies, we identify consensuses among studies with consistent findings and resolve conflicts among contradictory ones. Our work contextualizes and unifies existing research streams which aim at explaining the cross-lingual potential of MLLMs. This review provides, first, an aligned reference point for future research and, second, guidance for a better-informed and more efficient way of leveraging the cross-lingual capacity of MLLMs.

==> Tables/Table_LexicalOverlap.tex <==
\begin{tabular}{lp{4cm}p{6cm}p{1cm}}
\hline
\textbf{Paper} & \textbf{Task} & \textbf{Model} & \textbf{Lang. type} \\
\hline
\citep{pires_how_2019} & POS & mBERT & NL \\
\citep{wu_beto_2019} & DC, NER, DP, NLI, POS & mBERT & NL \\
\citep{tran_zero-shot_2019} & DP & mBERT & NL \\
\citep{lin_choosing_2019} & DP, MT, POS & / & NL \\
\citep{k_cross-lingual_2020} & NLI, NER & Bilingual BERT & NL/SL \\
\citep{conneau_emerging_2020} & NLI, NER, DP & Bilingual BERT & NL/SL \\
\citep{srinivasan2021} & NER, POS, NLI & mBERT, XLM-R & NL \\
\citep{de_vries_make_2022} & POS & XLM-R Base & NL \\
\citep{patil_overlap-based_2022} & NER, POS, DC, NLI & mBERT (12 languages) & NL/SL \\
\citep{deshpande_when_2022} & NLI, NER, POS, QA & Bilingual RoBERTa (small) & SL \\
\citep{ahuja_multi_2022} & DC, NLI, POS, NER, QA & mBERT, XLM-R & NL \\
\hline
\end{tabular}






%\begin{tabular}{lp{4cm}p{6cm}p{1cm}}
%\hline
%\textbf{Paper} & \textbf{Task} & \textbf{Model} & \textbf{Language type} \\
%\hline
%\citep{pires_how_2019} & \underline{POS}, NER & mBERT Base cased & NL \\
%\citep{wu_beto_2019} & \textbf{DC}, \textbf{NER}, \underline{DP}, \textit{NLI}, \underline{POS} & mBERT Base cased & NL \\
%\citep{tran_zero-shot_2019} & \textit{DP} & mBERT Base cased & NL \\
%\citep{lin_choosing_2019} & \underline{DP}, \underline{MT}, \underline{POS}, \st{Entity Linking} & / & NL \\
%\citep{k_cross-lingual_2020} & \textit{NLI}, \textit{NER} & Bilingual BERT & NL/SL \\
%\citep{conneau_emerging_2020} & \textit{NLI}, \textit{NER}, \textit{DP} & Bilingual BERT & NL/SL \\
%\citep{srinivasan2021} & \textbf{NER}, \underline{POS}, \textit{NLI} & mBERT, XLM-R Large & NL \\
%\citep{de_vries_make_2022} & \textit{POS} & XLM-RoBERTa Base & NL \\
%\citep{patil_overlap-based_2022} & \textbf{NER}, \underline{POS}, \textbf{DC}, \underline{NLI} & mBERT Base (12 langs?) & NL/SL \\
%\citep{deshpande_when_2022} & \underline{NLI}*, \underline{NER}*, \underline{POS}*, \underline{QA}* & Bilingual RoBERTa (small variant) & SL \\

%\citep{ahuja_multi_2022} & \textbf{DC}, \textbf{NLI}, \underline{POS}, \underline{NER}, \textbf{QA} & mBERT Base cased, XLM-RoBERTa Large & NL \\
%\hline
%\end{tabular}

==> Tables/Table_ModelArchitecture.tex <==
\begin{tabular}{lll}
\hline
\textbf{Paper} & \textbf{Task} & \textbf{Model}\\
\hline
\citep{k_cross-lingual_2020} & NLI, NER & Bilingual BERT \\
\citep{conneau_emerging_2020} & NLI, NER, DP & Bilingual BERT \\
\citep{dufter_identifying_2020} & NLI & BERT (small) \\
\citep{wu2022} & SA, AJ, SS, NLI & English RoBERTa \\
\citep{deshpande_when_2022} & NLI, NER, POS, QA & Bilingual RoBERTa (small) \\
\hline
\end{tabular}


==> Tables/Table_PreTrainData.tex <==
\begin{tabular}{lll}
\hline
\textbf{Paper} & \textbf{Task} & \textbf{Model}\\
\hline
\citep{lin_choosing_2019} & DP, MT, POS, EL & / \\
\citep{lauscher_zero_2020} & DP, POS, NER, NLI, QA & mBERT, XLM-R \\
\citep{liu2020} & NLI & mBERT \\
\citep{dufter_identifying_2020} & WA, WT, SR & mBERT (small) \\
\citep{conneau_emerging_2020} & NLI, NER, DP & Bilingual BERT \\
\citep{srinivasan2021} & NLI, NER, POS & mBERT, XLM-R \\
\citep{deshpande_when_2022} & NLI, NER, POS, QA & Bilingual RoBERTa (small) \\
\citep{ahuja_multi_2022} & DC, NLI, POS, NER, QA & mBERT Base cased, XLM-R \\
\hline
\end{tabular}






==> Tables/Table_PreTrainSettings.tex <==
\begin{tabular}{lll}
\hline
\textbf{Paper} & \textbf{Task} & \textbf{Model}\\
\hline
\citep{k_cross-lingual_2020} & NLI, NER & Bilingual BERT \\
\citep{artetxe_cross-lingual_2020} & NLI, DC, QA &  Bilingual BERT, mBERT \\
\citep{liu2020} & NLI & mBERT \\
\citep{ahuja_multi_2022} & DC, NLI, POS, NER, QA & mBERT, XLM-R \\
\hline
\end{tabular}




